Exploring the Potential of the Pulsed Laser onboard the CALIPSO Satellite to Improve Calibration with VERITAS

Imaging Atmospheric Cherenkov Telescopes (IACTs) are used to detect bright nanosecond-duration flashes of optical light originating from interactions of cosmic/gamma-rays in the atmosphere. A natural calibration source with similar characteristics does not exist; however, satellite-based laser systems provide a potential alternative. The CALIPSO satellite is one such facility which uses a suite of instruments to gather information about the atmosphere. Of particular interest is the CALIOP instrument, which emits 20-nanosecond laser pulses at 1064 nm and 532 nm at a rate of 20 Hz towards the Earth. The TAIGA-HiSCORE collaboration announced a detection of CALIOP laser pulses at the 37th ICRC in 2021, demonstrating that the laser footprint extends to at least tens of kilometers from the subsatellite point. We have used the VERITAS IACT to observe CALIPSO, and show here the results of using these observations to help to calibrate the array. We also discuss the potential of this technique for cross-calibration between different IACT facilities and for relative calibration between the telescopes of future large arrays.

==> table.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|} 
\hline Telescope ID & Current & This Analysis \\ 
\hline 1 & $0.$ & $0. \pm 0.077$ \\ 
\hline 2 & $0.612$ & $0.692 \pm 0.092$ \\ 
\hline 3 & $-0.806$ & $-0.426 \pm 0.088$ \\ 
\hline 4 & $2.027$ & $2.086 \pm 0.079$ \\ 
\hline 
\end{tabular}
\caption{Table of the measured rotations from this analysis and the rotation measurements currently used in VERITAS. The rotations have been modified from their original values to be relative to Telescope 1 for ease of comparison; all measurements are in degrees.}
\label{table:rotation_results}
\end{table}

